Code-Survey: An LLM-Driven Methodology for Analyzing Large-Scale Codebases

Modern software systems like the Linux kernel are among the world's largest and most intricate codebases, continually evolving with new features and increasing complexity. Understanding these systems poses significant challenges due to their scale and the unstructured nature of development artifacts such as commits and mailing list discussions. We introduce Code-Survey, the first LLM-driven methodology designed to systematically explore and analyze large-scale codebases. The central principle behind Code-Survey is to treat LLMs as human participants, acknowledging that software development is also a social activity and thereby enabling the application of established social science techniques. By carefully designing surveys, Code-Survey transforms unstructured data, such as commits, emails, into organized, structured, and analyzable datasets. This enables quantitative analysis of complex software evolution and uncovers valuable insights related to design, implementation, maintenance, reliability, and security. To demonstrate the effectiveness of Code-Survey, we apply it to the Linux kernel's eBPF subsystem. We construct the Linux-bpf dataset, comprising over 670 features and 16,000 commits from the Linux community. Our quantitative analysis uncovers important insights into the evolution of eBPF, such as development patterns, feature interdependencies, and areas requiring attention for reliability and security. The insights have been initially validated by eBPF experts. Furthermore, Code-Survey can be directly applied to other subsystems within Linux and to other large-scale software projects. By providing a versatile tool for systematic analysis, Code-Survey facilitates a deeper understanding of complex software systems, enabling improvements across a variety of domains and supporting a wide range of empirical studies. The code and dataset is open-sourced.

==> case-study_old.tex <==
\section{Case Study: eBPF}

In this section, we apply the \emph{Code-survey} methodology to analyze the evolution and development of the eBPF subsystem in the Linux kernel. We aim to uncover deep insights into the life cycle, stability, and design decisions of key eBPF features. The results generated by the survey are validated through expert review, as well as quantitative and qualitative analysis.

The Extended Berkeley Packet Filter (eBPF)\cite{ebpf} is a rapidly evolving subsystem in the Linux kernel that allows users to run sandboxed programs in kernel space without modifying the kernel itself \cite{lim2024safebpf}. Originally developed for packet filtering, eBPF now supports diverse use cases like performance tracing, security monitoring, and system observability, and also expand to multiple platforms\cite{windows-ebpf, zheng2023bpftime}. The academic also identifies the current problem and limitation of eBPF, and proposes several works to improve the verifier, deployment.


\subsection{Motivation: Features in eBPF Kernel with Data Analysis}

Let's see how traditional data analysis can bring. With traditional methods and well-defined kernel commits, we can analyze the eBPF kernel feature datasets to study the evolution of various eBPF features, such as helpers, maps, attach types, and other functionalities. We obtained the feature pairs from eBPF-docs\cite{ebpfdocs}, and combined them with Git commit data.

\subsubsection{How Do All eBPF Features Evolve Over Time?}

\Cref{fig:cumulative_feature_timeline} shows trends in the adoption of new features on the overall eBPF subsystem.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{feature-analysis/cumulative_bpf_features_timeline.png}
    \caption{Cumulative eBPF Features Timeline}
    \label{fig:cumulative_feature_timeline}
\end{figure}

\paragraph{Key Takeaways:}

\begin{enumerate}
    \item \textbf{Helpers and kfuncs} show the most growth for different use cases and changes.
    \item \textbf{Other features} see steady increases in the past 4 years, indicating their maturity.
\end{enumerate}

\subsubsection{Timeline of eBPF Helper Functions vs.\ Kernel Functions}

\Cref{fig:cumulative_helper_kfunc_timeline} shows the evolution of eBPF helper functions and kfuncs over time. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{feature-analysis/cumulative_helper_kfunc_timeline.png}
    \caption{Cumulative Helper and kfunc Timeline}
    \label{fig:cumulative_helper_kfunc_timeline}
\end{figure}

\paragraph{Key Takeaways:}

\begin{enumerate}
    \item \textbf{Helper functions} have been stable since 2023, and almost no new helpers are being added.
    \item \textbf{kfuncs} are growing very rapidly, showing the community's interest in expanding kernel interaction via kfuncs.
    \item All new use cases now tend to use \textbf{kfuncs} to influence kernel behavior, signaling a shift towards deeper kernel integrations.
\end{enumerate}

\subsubsection{What Are the Patterns in Other eBPF Features?}

\Cref{fig:cumulative_without_helper_timeline} examines eBPF feature evolution, excluding helpers and kfuncs. The focus is on core eBPF features and their impact on the overall subsystem.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{feature-analysis/cumulative_bpf_features_timeline_no_helper_kfunc.png}
    \caption{Cumulative eBPF Features Timeline Without Helpers and kfuncs}
    \label{fig:cumulative_without_helper_timeline}
\end{figure}

\paragraph{Key Takeaways:}

\begin{enumerate}
    \item \textbf{Core features} like events, flags, map types, and program types have stabilized after 2020.
    \item The introduction of \texttt{bpf\_link} greatly helps manage growing use cases and complexity, shows a significant difference before and after introduced.
\end{enumerate}

\paragraph{However\ldots}

The analysis of eBPF features mainly relies on kernel structured definitions and data sources obtained by humans, which is limited by the availability of data, and the time-consuming process of manual data collection.

There are massive amounts of unstructured data in the form of commit messages, code changes, and developer discussions that can provide valuable insights into the evolution and design decisions of eBPF features. While it is possible for humans to perform empirical analysis on some of this data, covering all of it is practically \emph{impossible}.

\textbf{Can AI assist us?} Instead of letting large language models (LLMs) attempt kernel coding, relying on retrieval-augmented generation (RAG) and fine-tuning to answer questions or code-review—which may yield incorrect answers—we propose a different quantitative approach.

By carefully designing a \emph{survey} and utilizing LLMs to \emph{transform} unstructured data like commits and emails into well-organized, structured, and easy-to-analyze datasets, we can perform \textbf{quantitative} analysis using traditional methods. In this way, AI can help analyze data and provide answers quickly; this capability is already a feature of platforms like ChatGPT.

\subsection{Research Questions for Survey Evaluation}

How can we ensure LLM is not answer questions randomly? To evaluate the effectiveness and correctness of the \emph{Code-survey} results, we explore the following high-level research questions:

\begin{itemize}
    \item \textbf{Correctness of Survey Responses:} How can we ensure that survey responses reflect accurate and relevant information about the system's features and commits?
    \item \textbf{Consistency Across Similar Questions:} Are similar questions answered consistently across different but related features or subsystems?
    \item \textbf{Coverage of Survey Questions:} Do the survey questions comprehensively cover all relevant aspects of the feature or subsystem under analysis?
    \item \textbf{Insight from Survey:} Can the survey data help user analysis the design, implementation, maintenance, reliability and security evlovment and gain valuable insights?
    \item \textbf{Clarity and Ambiguity in Responses:} Are the survey responses clear and unambiguous, making them actionable for further analysis?
    \item \textbf{Alignment with Real-World Changes:} How accurately do survey results reflect real-world changes in the software’s features and evolution?
    \item \textbf{Expert Confirmation:} How do experts rate the accuracy of the survey's generated insights?
\end{itemize}

\subsection{Commit Survey Design and Objectives}

To gain deeper insights into the design and evolution of the eBPF subsystem, we first developed a comprehensive survey aimed at classifying commits within the Linux eBPF subsystem. This survey evaluates specific aspects of each commit by analyzing commit messages and associated code changes. In cases where the commit message provides insufficient information, respondents are allowed to select an "I'm not sure" option.

The primary goals of the survey are to:

\begin{itemize} \item Provide concise summaries of each commit. \item Extract key themes and components affected by each commit. \item Classify commits based on their type, complexity, and impacted components. \item Identify patterns and trends in the evolution of the eBPF subsystem. \end{itemize}

\subsubsection{Survey Structure}

The survey consists of a series of structured questions designed to capture the essential characteristics of each commit. Respondents are encouraged to be as specific as possible based on the available commit message and code changes. If the commit message lacks clarity, the "I'm not sure" option can be selected.

\subsubsection{Simplified Survey Definition}

Below is the simplified survey structure:

\begin{enumerate}
    \item \textbf{Summary}: Provide a one-sentence summary of the commit (max 30 words).
    \item \textbf{Keywords}): Extract up to three keywords from the commit.
    \item \textbf{Commit Classification} (\emph{Single Choice}): What is the main type of the commit?
    \begin{enumerate}[label=(\alph*)]
        \item Bug fix
        \item New feature
        \item Performance optimization
        \item Code cleanup or refactoring
        \item Documentation change or typo fix
        \item Test case or test infrastructure change
        \item Build system or CI/CD change
        \item Security fix
        \item Merge commit
        \item Other type of commit
        \item I'm not sure
    \end{enumerate}
    \item \textbf{Commit Complexity} (\emph{Single Choice}): Estimate the complexity of implementing this commit.
    \begin{enumerate}[label=(\alph*)]
        \item Simple (affects 1--20 lines or 1--2 files)
        \item Moderate (affects 21--100 lines or a few files)
        \item Complex (affects over 100 lines or 5+ files)
        \item Merge-like (merges multiple branches or features)
        \item Non-code or generated changes
        \item I'm not sure
    \end{enumerate}
    \item \textbf{Major Related Implementation Component} (\emph{Single Choice}): What is the main implementation component modified?
    \begin{enumerate}[label=(\alph*)]
        \item eBPF verifier
        \item eBPF JIT compiler
        \item Helpers and kfuncs
        \item Syscall interface
        \item eBPF maps
        \item \texttt{libbpf} library
        \item \texttt{bpftool} utility
        \item Test cases and makefiles
        \item Changes in other subsystems related to eBPF events
        \item Merge commit
        \item Other component related to eBPF
        \item Unrelated to eBPF subsystem
        \item I'm not sure
    \end{enumerate}
    \item \textbf{Major Related Logic Component} (\emph{Single Choice}): What is the main logic component affected?
    \begin{enumerate}[label=(\alph*)]
        \item eBPF instruction logic
        \item Runtime features logic
        \item eBPF events-related logic
        \item Control plane interface logic
        \item Maps logic
        \item BPF Type Format (BTF) logic
        \item Merge commit
        \item General utilities logic
        \item Other eBPF logic component
        \item Unrelated to eBPF subsystem
        \item I'm not sure
    \end{enumerate}
    \item \textbf{Use Cases or Submodule Events} (\emph{Multiple Choice}): What eBPF use cases or subsystem events does the commit relate to?
    \begin{enumerate}[label=(\alph*)]
        \item XDP-related programs
        \item Socket-related programs
        \item \texttt{tc}-related programs
        \item Netfilter-related programs
        \item Tracepoints-related programs
        \item Kernel probes (\texttt{kprobe}/\texttt{ftrace})
        \item User-space probes (\texttt{uprobe}/USDT)
        \item Profiling-related programs
        \item LSM-related programs
        \item \texttt{struct\_ops}-related programs
        \item \texttt{cgroup}-related programs
        \item HID driver-related programs
        \item Scheduler-related programs
        \item Improves overall eBPF infrastructure
        \item Merge commit
        \item Other eBPF use cases
        \item Unrelated to eBPF subsystem
        \item I'm not sure
    \end{enumerate}
\end{enumerate}

% \subsubsection{Survey Implementation Notes}

% The goal of transforming unstructured data (commit messages and code changes) into structured responses is to facilitate quantitative analysis of the evolution of the eBPF subsystem. The survey is designed to capture key attributes of each commit, enabling the identification of patterns, trends, and areas that require significant development or maintenance effort.

% For each question, respondents should:

% \begin{itemize} \item Be as specific as possible based on the commit message and code changes. \item Select the "I'm not sure" option if the information is insufficient. \item Recognize that some commits may affect multiple components or use cases. \end{itemize}

\subsection{Implementing the Survey Using LLM Agent}

To efficiently process and analyze the vast number of commits in the Linux eBPF subsystem, we leveraged Large Language Models (LLMs), to automate our survey. We develop a Assistant Agent in GPTs\cite{gpts} for Generating Survey, and a Assistant Agent to help analysis results. By utilizing gpt4o\cite{gpt4o} LLM model, we transformed unstructured commit data into structured responses aligned with our survey definitions. We first conduct the method on 15000+ commits across 8 years, and plan to expand it to the mails and patches.

\subsubsection{Commit Survey Methodology}

Our first simple approach uses an AI model to analyze each commit's details and answer the survey questions. The process includes:

\begin{enumerate} 
\item \textbf{Data Extraction}: We gather key commit details such as commit ID, author info, commit date, message, code changes, and mails. 
\item \textbf{Prompt Construction}: A prompt containing the survey title, description, change files, and commit details is generated to guide the AI.
\item \textbf{AI Model Interaction}: The AI processes the prompt, analyzing the commit message and code changes to respond to the survey. For each commit, The AI receives the commit details and survey questions, completes them, and generates struct output as a JSON.
\item \textbf{Feedback Loop}: If the AI's response is incomplete or inconsistent, it re-evaluates and revises the answers to improve accuracy.
\item \textbf{Data Aggregation}: The AI’s responses are stored for later quantitative analysis. 
\end{enumerate}

We used the GPT-4o model for its strong language understanding and ability to handle technical content, making it well-suited for analyzing kernel commits.

\subsubsection{Enhancing Survey Accuracy}

Due to the limitation of time and budget, the performance of AI in this experiment can still be greatly improved. Several strategies can improve accuracy:

\begin{itemize} 
\item \textbf{Multiple Iterations}: Running the survey multiple times and averaging results, similar to human surveys, can significantly reduce response variability. Due to budget limits, we ran it once per commit, and the results are already meaningful with <1\% error. We plan to running the survey multiple times and have a better evaluation in the future work.
\item \textbf{Advanced Models}: Fine-tuning domain-specific LLMs for kernel development, or better models like o1\cite{o1} can capture technical nuances better. 
\item \textbf{Refined Prompt Engineering}: Crafting clearer prompts and survey questions will improve response accuracy. 
\item \textbf{Multi-Step Reasoning}: Using multi-step processes or multi-agent systems can also help analyze complex commits more thoroughly. 
\end{itemize}

Automating the survey with LLM enabled us to efficiently process tens of thousands of commits, transforming unstructured data into structured insights.

\subsection{The Commit Dataset}

The \texttt{commit\_survey.csv} dataset provides detailed metadata for over 15,000 Linux kernel commits, including commit types, messages, timestamps, and affected components. It is used to categorize and classify commits, focusing on the eBPF subsystem.

\subsubsection{Dataset Overview}
The dataset contains the following fields:
\begin{itemize}
    \item \textbf{Commit Metadata}: Unique commit IDs, author, committer details, and timestamps.
    \item \textbf{Commit Messages and file changes}: Descriptions of the changes in each commit.
    \item \textbf{Classification}: Types such as bug fixes, feature additions, or merges.
    \item \textbf{Complexity}: Based on file and line changes.
    \item \textbf{Components}: Affected implementation and logic components.
    \item \textbf{Use Cases}: Related subsystems and modules.
\end{itemize}

\subsubsection{Distribution of dataset}

\paragraph{Commit Classification Distribution}
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{feature-analysis/commit_pie_chart_commit_classification.png}
    \caption{Commit Classification Distribution}
    \label{fig:commit_pie_chart_commit_classification}
\end{figure}

Most commits are focused on bug fixes and cleanups, reflecting efforts to maintain code quality. Testing infrastructure changes are also significant, showing the emphasis on robustness. New features make up a large portion of the commits, while merge commits are typical in the Linux kernel.

\paragraph{Commit Complexity Distribution}
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{feature-analysis/commit_pie_chart_commit_complexity.png}
    \caption{Commit Complexity Distribution}\label{fig:commit_pie_chart_commit_complexity}
\end{figure}

The majority of commits are simple, involving small changes, while more complex changes make up a smaller, but notable, portion.
\paragraph{Major Related Implementation Components}
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{feature-analysis/commit_pie_chart_major_implementation_component.png}
    \caption{Major Related Implementation Components}\label{fig:commit_pie_chart_major_implementation_component}
\end{figure}

Test cases and build scripts are significantly impacted, highlighting continuous improvements in testing and build processes. \texttt{libbpf} is also a key component in the kernel eBPF toolchain. Additionally, a large amount of development occurs in other kernel subsystems, particularly in relation to eBPF events. The frequency of updates to the eBPF verifier and helpers also indicates ongoing efforts to enhance functionality and ensure program safety. Notably, some commits seems not related to eBPF subsystems.

\paragraph{Logic Components Affected}
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{feature-analysis/commit_pie_chart_major_logic_component.png}
    \caption{Major Related Logic Components}
\end{figure}

General utilities, such as tools and scripts, see the most updates, followed by runtime features like helpers and kernel functions, which are consistently enhanced. eBPF event logic and instruction handling are also frequently updated to ensure robustness and functionality.
 
\paragraph{Use Cases and eBPF Events}
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{feature-analysis/commit_pie_chart_usecases_or_submodule_events.png}
    \caption{Related Events and Use Cases}
\end{figure}

While most commits enhance core eBPF infrastructure, including the verifier and runtime components, their development 
Networking-related features, such as socket and XDP programs, receive significant attention, while tracing tools like tracepoints and kprobes show eBPF's important role in system diagnostics and debugging.

\subsection{Correctness of Survey Responses}

To ensure survey responses accurately reflect system features and commits, we validate responses by randomly sampling the data and cross-referencing with expert knowledge and processing logs. Specifically, we addressed two common issues: the handling of merge commits and the identification of commits unrelated to the BPF subsystem.

\subsubsection{Merge Commit Correctness}

For merge commits, we observed a discrepancy between the commit classification perspective and the major implementation component perspective.  To address this, we analyzed the top merge commit messages and determined that some merge commits were categorized based on their predominant effect on a specific component rather than being uniformly labeled as merge commits. By making this clear in the survey questions, we ensured that the survey's classification system accounted for these distinctions and reflected the correct commit impact across perspectives.

\textbf{Example:}
\begin{verbatim}
Top Commit (Classification but not Implementation):
3    Merge branch 'bpf-fix-incorrect-name-check-pass'
25   Merge branch 'vsc73xx-fix-mdio-and-phy' Pawel...
\end{verbatim}

\subsubsection{Non-Related BPF Subsystem Commits}

We noted that commits not directly related to the BPF subsystem were sometimes included due to broad filtering criteria (e.g., \textbf{--grep=bpf}). After reviewing these commits, we confirm some commits mentioned "bpf" but addressed unrelated or peripheral issues.

\textbf{Example:}
\begin{verbatim}
Sample 'Not related to BPF' Commit Messages:
17    bonding: fix xfrm real_dev null pointer...
21    btrfs: fix invalid mapping of extent xarray st...
\end{verbatim}

\subsubsection{Consistency Across Similar Questions}

We checked for consistency in responses by comparing related questions, focusing on the merge commit numbers in commit classifications and complexities, and also unrelated components commit numbers in Implementation and logic components.

\textbf{Example 1: Merge Commits}
\begin{itemize}
    \item \textbf{Commit Classification:} "It's like a merge commit." (1,347 responses)
    \item \textbf{Commit Complexity:} "Merge-like. The commit merges branches." (1,346 responses)
\end{itemize}

\textbf{Example 2: Unrelated Components}
\begin{itemize}
    \item \textbf{Implementation Component:} "Not related to BPF." (606 responses)
    \item \textbf{Logic Component:} "Not related to BPF." (602 responses)
\end{itemize}

The close match shows consistent identification of unrelated components. With a low misclassification rate (under 0.05\%), our data shows high consistency, supporting the reliability of the survey design.

\subsection{Timeline Analysis of Commits}

The timeline analysis of commits offers valuable insights into the evolution of the eBPF subsystem over time. By visualizing the distribution of commit types, complexities, and major components across different periods, trends and patterns in the development of eBPF features become evident.

The data was processed by cleaning it to remove irrelevant commits, smoothing it using a 3-month average to reduce noise and highlight long-term trends, and treating single-component \texttt{Merge} commits as regular commits while removing multi-component \texttt{Merge} commits, such as mainline merges. The time span is from 2017 to the end of 2024, with more than 15000 commits.

\subsubsection{Commit Classification Over Time}
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{feature-analysis/timeline_commit_classification_smoothed.png}
    \caption{Commit Classification Over Time}\label{fig:timeline_commit_classification_smoothed}
\end{figure}
\Cref{fig:timeline_commit_classification_smoothed} shows the distribution of different types of code commits over time.

The development started to grow significantly in 2017, but the addition of test cases was limited at first and continued to improve later. New feature development follows a cyclical pattern, with notable spikes around 2020 and 2021. After 2021, the number of cleanups and refactoring increases significantly, while new feature additions decline, indicating a shift in focus towards code maintainability and stability. A decline of cleanup commits after 2023 suggests that while new features continue to be added, the focus has shifted more towards stabilization and optimization.

\subsubsection{Commits Related to Major Implementation Components Over Time}
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{feature-analysis/timeline_major_related_implementation_component_smoothed.png}
    \caption{Commits Related to Major Implementation Components Over Time}\label{fig:timeline_major_related_implementation_component_smoothed}
\end{figure}

\Cref{fig:timeline_major_related_implementation_component_smoothed} shows the evolution of major implementation components in the Linux BPF subsystem.

Most components see their highest activity between 2017 and 2022, reflecting the rapid development of eBPF features during this time. The libbpf library saw the most dramatic increase, while the JIT compiler was most frequently updated around 2018. The rise in test cases also reflects the growing importance of a robust testing framework being introduced in this field.

After peaking around 2021-2022, several components show a decline or stabilization in activity. This indicates that many eBPF components have entered a phase of optimization and maintenance rather than new feature development, while testing continues to be applied to increase coverage. The verifier shows modest activity throughout the observed period but seems to increase in 2023-2024, which may reflect renewed research efforts in this area.
 
\subsubsection{Commit Related to Major Logic Component Over Time}
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{feature-analysis/timeline_major_related_logic_component_smoothed.png}
    \caption{Commit Related to Major Logic Components Over Time}\label{fig:timeline_major_related_logic_component_smoothed}
\end{figure}
\Cref{fig:timeline_major_related_logic_component_smoothed} depicts the evolution of major logic components in Linux BPF subsystem. 

Figure \ref{fig:timeline_major_related_logic_component_smoothed} shows the number of commits for various logic components or features. Most improvements are around The general utilities" component, which peaks around 2022-2023 before decreasing. Other components like "Runtime features, helpers and kfuncs" and "eBPF Instruction Logic" show more gradual increases over time, while components such as "Control Plane interface" and "Maps Logic" maintain relatively steady levels of activity throughout the period.

\subsubsection{Use Cases or Events Over Time}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{feature-analysis/timeline_usecases_or_submodule_events_smoothed.png}
    \caption{Use Cases or Events Over Time }\label{fig:timeline_usecases_or_submodule_events_smoothed}
\end{figure}

\Cref{fig:timeline_usecases_or_submodule_events_smoothed} reveals significant fluctuations in event types over the years.

The most notable are the network-related events, such as socket and XDP programs. There was a surge in both socket- and XDP-related activities from 2020 to 2022, after which they entered a stabilization phase following the initial burst of feature additions and optimizations. The tracepoints-related line shows a steady increase with periodic fluctuations, peaking around 2021 before decreasing. The kprobe/ftrace-related events remain mostly stable, with a slight increase in 2022. uprobe-related events show moderate activity over several years, with a slight peak in 2022 and again in 2024. Struct\_ops, an emerging feature introduced in 2020, shows a significant increase in activity between 2023 and 2024. Other events such as LSM for security are still minor.

\subsection{Deeper Insights Analysis}

This section delves into the survey responses to uncover patterns, trends, and areas for improvement within the eBPF subsystem.
\subsubsection{Which Kernel Components and Files Have the Most Frequent Bugs?}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{feature-analysis/commit_pie_buggy_kernel_componenet.png}
    \caption{Verifier Instruction Features vs. General Verifier Bugs Over Time}
    \label{fig:buggy_kernel_component}
\end{figure}

\Cref{fig:buggy_kernel_component} illustrates the kernel implementation components with a large number of bugs. While previous analyses and tools have primarily focused on improving the stability of the verifier and JIT compiler, these areas account for only about 35\% of the bugs. The largest amount of bugs originate from eBPF event-related code, which involves the interaction of eBPF with other kernel subsystems. Additionally, helpers and maps also have a significant number of bugs. Due to the complexity of the control plane, the syscall interface of eBPF is also prone to bugs.

By examining the specific files, we can also observe that bugs frequently occur in the verifier, syscall, core, and network filter components. The kernel needs better coverage and more attention on these files.

\textbf{Top 5 Buggy Files:}
\begin{verbatim}
 kernel/bpf/verifier.c             425
 net/core/filter.c                 140
 kernel/bpf/syscall.c              111
 include/linux/bpf.h                87
 kernel/bpf/core.c                  83
\end{verbatim}


\subsubsection{What is the Relationship Between Instruction-Related Changes in the Verifier and All Verifier Bugs?}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{feature-analysis/instruction_verifier_features_bugs_over_time.png}
    \caption{Verifier Bugs or Features Related to eBPF Instruction Over Time}
    \label{fig:instruction_verifier_features_bugs_over_time}
\end{figure}

\Cref{fig:instruction_verifier_features_bugs_over_time} shows that changes related to eBPF instructions in the verifier are closely related to the number of verifier bugs. This insight highlights the importance of focusing on instruction-related aspects during verifier development and debugging to enhance overall system stability.

\subsubsection{The Evolution and Status of libbpf}

We also examined the lifecycle of specific components, such as \texttt{libbpf}.

Based on \Cref{fig:libbpf_commit_classification}, the development of libbpf began to grow significantly in 2017. New feature development follows a cyclical pattern, with notable spikes around 2020 and 2022. After 2022, the number of cleanups and refactorings increased significantly, indicating a shift in focus towards code maintainability and stability. However, the decline in cleanup commits after 2023 suggests that while new features continue to be added, the focus has shifted more towards stabilization and optimization.

Historical milestones verify this trend. For instance, libbpf version 1.0 was released in August 2022 \cite{libbpf1}, and the major feature "Compile Once, Run Everywhere" (CO-RE) was introduced around 2020 \cite{core}, both aligning with the peaks and shifts observed in the commit history.


\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{feature-analysis/timeline_libbpf_commit_classification_smoothed.png}
    \caption{Evolution of \texttt{libbpf} Over Time}
    \label{fig:libbpf_commit_classification}
\end{figure}

\subsection{Expert Confirmation} 

We discussed the results with more than five eBPF experts who have submitted kernel patches or given conference talks. They confirmed that the results are likely correct based on their understanding. We also shared the report with kernel maintainers and the BPF kernel mailing list, which is under discussion. Additionally, we plan to provide experts with a sample of survey responses and ask them to rate the accuracy of each response on a defined scale. Based on their feedback, we will refine the survey to improve its correctness and relevance.

\subsection{Clarity and Ambiguity in Responses}

Based on the insights gathered from the survey responses, the survey results are likely clear and  actionable. We plan to invite more experts to review a sample of the responses to identify any vague or unclear answers. Afterward, we will revise any survey questions prone to misinterpretation or ambiguity to improve clarity and precision.

\subsection{Alignment with Real-World Changes}

By compare survey responses with real-world feature changes discussed before, we confirm that the survey likely captures the correct historical context. We plan to cross-reference survey results with commit histories, mailing list discussions, and kernel release notes to further verify alignment with real-world changes.


\subsection{Coverage of Survey Questions}

We plan to review the survey’s coverage to identify potential gaps, ensuring that important aspects such as security, performance, and dependencies are addressed.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{feature-analysis/cumulative_bpf_features_timeline.png}
%     \caption{Cumulative bpf features timeline}
%     \label{fig:feature}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{feature-analysis/timeline_major_related_implementation_component_smoothed.png}
%     \caption{Timeline major related implementation component smoothed}
%     \label{fig:smoothed}
% \end{figure}

==> intro_old.tex <==
% \begin{IEEEkeywords}
% LLM
% \end{IEEEkeywords}

% \section{Introduction}
% % \begin{figure}[t]
% % \centering
% % \includegraphics[width=0.9\linewidth]{00A9.png}
% % \caption{
% % placeholder
% % }
% % \label{fig:adaptation}
% % \end{figure}
% Software systems are growing increasingly complex, with real-world applications often requiring continuous development over time. Unlike research projects, where goals are clearly defined and the development process is relatively controlled, real-world systems evolve organically. Features are added incrementally, bugs are fixed, and design decisions are sometimes modified years after the initial development. This complexity is exacerbated by the need to balance backward compatibility, feature requests, performance improvements, and security patches. As systems evolve, it becomes difficult to trace the original intent behind design decisions or understand the rationale behind modifications. This lack of transparency in the development process often leads to issues such as technical debt, regressions, and challenges in maintaining system reliability.

% One of the most prominent examples of a continuously evolving, real-world system is the Linux kernel. As the backbone of countless devices and platforms, from cloud servers to mobile devices, the Linux kernel must support a wide array of features and maintain rigorous performance standards. Take eBPF subsystem as an example. The \textit{extended Berkeley Packet Filter}\cite{ebpf} (eBPF) subsystem is a prime example of the complexity within Linux, as it supports critical functionalities such as observability\cite{shen2023network}, networking\cite{vieira2020fast} and security\cite{deri2019combining}. However, despite its significance, much of the development history and design rationale behind eBPF remains underexplored. Features like \texttt{bpf\_link}\cite{bpflink}, which allow various components to interact within the kernel, have been part of the Linux source code for several years but receive little attention outside kernel developers. The increasing use of kfuncs\cite{kfuncs} in place of helpers, along with the growing complexity of control-plane applications, has also received less attention.

% In general software development, understanding the evolution of features in large, complex codebases presents a significant challenge\cite{godfrey2008past, mens2008introduction}. Traditional methods, such as static analysis and manual code review, are limited in their ability to capture the full context of a system's growth and change, and require huge amount of human effort. Unstructured data sources, such as commit messages and mailing list discussions, contain valuable insights but are difficult to analyze systematically. As a result, important information about design decisions, feature evolution, and system behavior is often hidden within large, unstructured text, making it nearly impossible to answer questions such as: "Why was this feature added?", "How has this feature evolved?", or "What were the discussions that led to this change?"

% Recent advancements in artificial intelligence, particularly in large language models (LLMs), like GPT4o \cite{gpt4o} and O1~\cite{o1}, have opened new opportunities for addressing these challenges. LLMs have shown great promise in automating software engineering tasks such as code generation\cite{zheng2024kgent}, bug detection\cite{li2024enhancing}, debug\cite{chen2023teaching}, and error fixing \cite{deligiannis2023fixing}. However, most current applications of LLMs focus on well-defined tasks, like source code or documented APIs. Little work has been done to explore how LLMs can be applied to understand the long-term evolution of large-scale real-world software systems.

% In this paper, we introduce \emph{Code-survey}, a novel methodology that leverages LLMs to systematically transform unstructured data, such as commit histories and emails\cite{linux,tan2019communicate,schneider2016differentiating}, into structured data for analysis and provide insights. By focusing on the huge amount of text produced in software development, Code-survey enables us to answer questions that were previously impossible to tackle using only structured data in huge real-world systems. The data analysis in Code-survey allows us to explore questions like: 

% \begin{itemize}
%     \item "How do new feature introductions impact the stability and performance of existing kernel components?"
%     \item "Are there identifiable phases in the lifecycle of a feature, such as initial development, stabilization, and optimization?"
%     \item "How has the functionality of a specific eBPF feature, evolved over successive commits?"
%     \item "Which component and file in Linux kernel has the highest bug frequency?"
%     \item "What lessons can be learned from the development history of kernel eBPF that can be applied to improving other eBPF runtimes?"
% \end{itemize}

% To demonstrate the efficacy of Code-survey, we apply it to the \textit{Linux-bpf dataset}, which contains over 670 features, 15,000 commits, and 150,000 emails related to the development of the eBPF subsystem. Through this structured dataset, we uncover new insights into the design and evolution of features like \texttt{bpf\_link} and highlight trends that were previously hidden within the unstructured data. The insights has been initially confirmed by eBPF experts.

% The key contributions of this paper are as follows:
% \begin{itemize}
%     \item We introduce \emph{Code-survey}, the first novel methodology that leverages LLMs to transform unstructured data produced in softwar development into structured datasets with a survey, enabling systematic analysis of software evolution.
%     \item We present the \textit{Linux-bpf dataset}, a structured dataset of over 670 features, 15,000 commits and 150,000 emails related to the eBPF subsystem in the Linux kernel.
%     \item We apply the \emph{Code-survey} methodology to build an LLM-driven agent system, allowing us to perform systematic analysis on the \textit{Linux-bpf dataset}.
%     \item We demonstrate that \emph{Code-survey} methodology reveals new insights into the evolution of eBPF kernel features that is impossible to be uncovered using traditional methods. Using transitional data analysis methods in Survey and combined with Kernel Expert's domain knowledge, we also proved the data is mostly Consistent and Correctness.
%     \item We also identify and call attention to under-explored areas of the eBPF to support the various use cases with the help of \emph{Code-survey}, highlighting interesting research directions. 
% \end{itemize}

% The remainder of this paper is structured as follows. We review related work in Section II, followed by a detailed explanation of the Code-survey methodology in Section III. Section IV presents our analysis of the Linux-bpf dataset and the insights gained from it. Section V discusses the best practice when designing AI based survey, and Section VI, VII concludes with a discussion of the current limitations and future work. All the artifacts are open-sourced in \url{https://github.com/eunomia-bpf/code-survey}.

% \section{Introduction}

% Software systems are increasingly complex, with real-world applications often requiring continuous development over time. Unlike research projects with clearly defined goals and controlled development processes, real-world systems evolve organically. Features are added incrementally, bugs are fixed, and design decisions may be modified years after initial implementation. This complexity is further exacerbated by the need to balance backward compatibility, feature requests, performance improvements, and security patches. As systems evolve, tracing the original intent behind design decisions or understanding the rationale for modifications becomes difficult. This lack of transparency often leads to technical debt, regressions, and challenges in maintaining system reliability.

% One of the most prominent examples of a continuously evolving real-world system is the Linux kernel. Serving as the backbone of countless devices and platforms—from cloud servers to mobile devices—the Linux kernel must support a wide array of features while maintaining rigorous performance standards. The \textit{extended Berkeley Packet Filter} (eBPF)\cite{ebpf} subsystem exemplifies this complexity, as it supports critical functionalities such as observability\cite{shen2023network}, networking\cite{vieira2020fast}, and security\cite{deri2019combining}. Despite its significance, much of the development history and design rationale behind eBPF remains underexplored. Features like \texttt{bpf\_link}\cite{bpflink}, which enable interaction between various kernel components, have been part of the Linux source code for several years but receive little attention outside kernel developers. Similarly, the increasing use of kfuncs\cite{kfuncs} in place of helpers, and the growing complexity of control-plane applications, have received limited attention.

% Understanding the evolution of features in large, complex codebases is a significant challenge in software development\cite{godfrey2008past,mens2008introduction}. Traditional methods, such as static analysis and manual code review, are limited in capturing the full context of a system's growth and change, and require substantial human effort. Unstructured data sources, like commit messages and mailing list discussions, contain valuable insights but are difficult to analyze systematically. Consequently, important information about design decisions, feature evolution, and system behavior is often hidden within large volumes of unstructured text. This makes it nearly impossible to answer questions such as: ``Why was this feature added?'', ``How has this feature evolved?'', or ``What were the discussions that led to this change?''

% Recent advancements in artificial intelligence, particularly in Large Language Models (LLMs) like GPT-4\cite{gpt4o} and O1~\cite{o1}, have opened new opportunities to address these challenges. LLMs have shown great promise in automating software engineering tasks such as code generation\cite{zheng2024kgent}, bug detection\cite{li2024enhancing}, debugging\cite{chen2023teaching}, and error fixing\cite{deligiannis2023fixing}. However, most current applications of LLMs focus on well-defined tasks involving source code or documented APIs. Little work has explored how LLMs can be applied to understand the long-term evolution of large-scale, real-world software systems.

% In this paper, we introduce \emph{Code-survey}, a novel methodology that leverages LLMs to systematically transform unstructured data---such as commit histories and emails\cite{linux,tan2019communicate,schneider2016differentiating}---into structured data for analysis. **To the best of our knowledge, \emph{Code-survey} is the first methodology that leverages Large Language Models (LLMs) to transform unstructured software development data into structured datasets for systematic analysis.** By focusing on the vast amount of text produced during software development, Code-survey enables us to answer questions that were previously difficult to tackle using only structured data in large real-world systems. Through data analysis enabled by Code-survey, we can explore questions such as:

% \begin{itemize}
%     \item ``How do new feature introductions impact the stability and performance of existing kernel components?''
%     \item ``Are there identifiable phases in the lifecycle of a feature, such as initial development, stabilization, and optimization?''
%     \item ``How has the functionality of a specific eBPF feature evolved over successive commits?''
%     \item ``Which components or files in the Linux kernel have the highest bug frequency?''
%     \item ``What lessons can be learned from the development history of kernel eBPF that can be applied to improving other eBPF runtimes?''
% \end{itemize}

% To demonstrate the efficacy of Code-survey, we apply it to the \textit{Linux-bpf dataset}, which contains over 670 features, 15,000 commits, and 150,000 emails related to the development of the eBPF subsystem. Through this structured dataset, we uncover new insights into the design and evolution of features like \texttt{bpf\_link}, and highlight trends that were previously hidden within the unstructured data. These insights have been initially confirmed by eBPF experts.

% The key contributions of this paper are as follows:

% \begin{itemize}
%     \item We introduce \emph{Code-survey}, a novel methodology that leverages LLMs to transform unstructured data produced in software development into structured datasets via surveys, enabling systematic analysis of software evolution.
%     \item We present the \textit{Linux-bpf dataset}, a structured dataset comprising over 670 features, 15,000 commits, and 150,000 emails related to the eBPF subsystem in the Linux kernel.
%     \item We apply the \emph{Code-survey} methodology to build an LLM-driven agent system, allowing us to perform systematic analysis on the \textit{Linux-bpf dataset}.
%     \item We demonstrate that the \emph{Code-survey} methodology reveals new insights into the evolution of eBPF kernel features that are impossible to uncover using traditional methods. By combining traditional data analysis methods with kernel experts' domain knowledge, we also verified the consistency and correctness of the data.
%     \item We identify and highlight under-explored areas of eBPF to support various use cases with the help of \emph{Code-survey}, pointing out interesting research directions.
% \end{itemize}

% The remainder of this paper is structured as follows. We review related work in Section~\ref{sec:related}, followed by a detailed explanation of the Code-survey methodology in Section~\ref{sec:methodology}. Section~\ref{sec:analysis} presents our analysis of the Linux-bpf dataset and the insights gained from it. Section~\ref{sec:best_practices} discusses best practices when designing AI-based surveys. Sections~\ref{sec:limitations} and~\ref{sec:conclusion} conclude with a discussion of current limitations and future work. All artifacts are open-sourced at \url{https://github.com/eunomia-bpf/code-survey}.


==> limit-futurework-old.tex <==

\section{Best Practices in Code-Survey Method}

The Code-survey method, especially when integrated with large language models (LLMs), requires carefully designed practices in Survey to ensure the accuracy and relevance of responses. The key idea is, to just create the survey for humans and allow LLM to perform on it. You can easily apply other approaches.

Below are some of the best practices to achieve reliable results:

\begin{enumerate}
    \item \textbf{Use Pre-Defined Tags and Categories:} To avoid hallucination or random answers, it is crucial to provide structured, closed-ended questions. Pre-defined tags such as ``bug," ``new feature," or ``performance improvement" help standardize responses and reduce ambiguity.
    
    \item \textbf{Incorporate a LLM Agent workflow:} LLMs may need to review their answers multiple times to improve accuracy. Implementing some feedback loop, ReAct or CoT planning approaches with memory allows the model to re-evaluate the questions and select the most appropriate response, enhancing overall data quality.
    
    \item \textbf{Allow for ``I Don’t Know" Responses:} When the LLM encounters unfamiliar or complex questions, providing an option to answer ``I don’t know" prevents random or misleading responses. This is particularly useful when domain knowledge is limited or incomplete.
    
    \item \textbf{Pilot Testing and Iterative Refinement:} Prior to full deployment, conducting a pilot test helps identify potential issues with question clarity and LLM understanding. Iterative refinement of questions based on these trials ensures logical consistency and improves data reliability.
    
    \item \textbf{Consistency and Data Validation:} Post-survey, apply validation checks to ensure consistency across responses. Detecting and filtering out illogical or contradictory answers is essential to maintaining the integrity of the data set.
\end{enumerate}

By following these best practices, the Code-survey method can leverage LLMs effectively, mitigating the risks of hallucination and improving the reliability of responses in technical domains such as Linux kernel commit analysis.


\section{Limitations}

While \emph{Code-survey} offers significant advancements in analyzing the evolution of large software systems, it is not without limitations:

\begin{itemize}
    \item \textbf{Dependency on Data Quality}: The accuracy of \emph{Code-survey} is heavily reliant on the quality and completeness of the input data. Incomplete commit messages or fragmented email discussions can lead to gaps in the structured data, potentially obscuring important aspects of feature evolution.

    \item \textbf{LLMs can make mistakes, just like humans}: Although LLMs like GPT-4 are powerful, they are not infallible. Misinterpretations of commit messages or developer communications can result in inaccurate data structuring. However, this is not a problem—humans make mistakes too, and LLMs can be treated like inexperienced or untrained individuals in some cases. For example, LLMs may hallucinate, similar to how a graduate student might imagine or fill in gaps. They are more prone to filling survey responses randomly, answering questions too quickly without careful thought, or missing important details in the questions. To mitigate these issues, careful survey design is essential to guide the model’s responses more effectively. The same technology design for human survey can be directly applied to LLM surveys.

    \item \textbf{Human Expert Oversight Requirement}: The performance of Code-survey largely depends on the quality of the survey. Despite automation, human expertise remains essential for designing effective surveys, evaluating results, and ensuring the contextual relevance of the structured data. This dependency can limit the scalability of \emph{Code-survey} in scenarios where expert availability is constrained.
\end{itemize}

\section{Future Work}

\emph{Code-survey} shows great potential in organizing and analyzing unstructured software data, but several areas need improvement and expansion:

\subsection{Combining Linux eBPF Mails and Other Sources}

While the current focus is primarily on commit data, we plan to extend the approach to include Linux eBPF mailing lists and other relevant data sources. This expansion will allow a more complete understanding of feature lifecycles and development discussions, providing more robust insights into the design and maintenance process.

\subsection{Improved Evaluation of LLM-Generated Survey Data}

While LLMs like GPT-4o generate structured data from unstructured inputs, issues like hallucination remain. Future work will develop validation frameworks to improve accuracy, benchmark results against curated datasets, and involve human experts in refining LLM outputs.

\subsection{Performance Enhancement with LLM Agents}

The current proof-of-concept demonstrates automation but with sub optimal performance and accuracy. Future efforts will evaluate the performance of fully automate the process using more advanced models (e.g., o1) and multi-agent systems to improve the performance. Additionally, ensuring the structured data is compatible and usable with machine analysis tools is crucial.

\subsection{Application to Other Projects}

Though \emph{Code-survey} has focused on the Linux eBPF subsystem, the method is adaptable to any Linux subststems ot other projects like Kubernetes, LLVM, and Apache. Expanding to these repositories will test its scalability and versatility, requiring adjustments for different development practices.

\subsection{Direct Structuring of Code and Functions}

Currently, \emph{Code-survey} relies on commits and mailing lists. Future research will extend this to code and functions, turning technical elements into structured, query-able data or graphs with attributes. This will enable a large number of algorithms and queries to be performed on it and provide deeper insights into the actual software implementations and evolution.

\subsection{Integration of Additional Data Sources}

Future work will incorporate data from code reviews, issue trackers, and documentation to provide a fuller picture of feature evolution and development. This holistic approach will offer more detailed insights into the software development lifecycle.

By pursuing these improvements, \emph{Code-survey} aims to become a comprehensive tool for analyzing complex software systems, benefiting both developers and empirical software researchers.

